Impact of Discretization Noise of the Dependent variable on Machine Learning Classifiers in Software Engineering

Researchers usually discretize a continuous dependent variable into two target classes by introducing an artificial discretization threshold (e.g., median). However, such discretization may introduce noise (i.e., discretization noise) due to ambiguous class loyalty of data points that are close to the artificial threshold. Previous studies do not provide a clear directive on the impact of discretization noise on the classifiers and how to handle such noise. In this paper, we propose a framework to help researchers and practitioners systematically estimate the impact of discretization noise on classifiers in terms of its impact on various performance measures and the interpretation of classifiers. Through a case study of 7 software engineering datasets, we find that: 1) discretization noise affects the different performance measures of a classifier differently for different datasets; 2) Though the interpretation of the classifiers are impacted by the discretization noise on the whole, the top 3 most important features are not affected by the discretization noise. Therefore, we suggest that practitioners and researchers use our framework to understand the impact of discretization noise on the performance of their built classifiers and estimate the exact amount of discretization noise to be discarded from the dataset to avoid the negative impact of such noise.

==> exp.tex <==
This section describes our data collection process and introduces our framework.

\subsection{Data Collection}\label{data}

In this paper, we collect data based on two criteria:1) the dependent variable is continuous; 2) the dataset's dependent variable lacks a clear-cut threshold for discretization. Based on these two criteria, we collect 4 types of data (7 datasets): Q\&A websites data~\cite{wang2017}, Linux patch acceptance time (Patch) data~\cite{jiang2013will}, Bug-fix delay time (Bug-delay) data~\cite{zhang2012empirical}, and Mobile app rating (App-rating) data~\cite{Tian:2015}. Table~\ref{tab:framework_tab_1} contains basic information about the number of data points and the independent features of each of the studied datasets.

%\begin{table}
%
%    \caption{Basic information about the studied datasets}\label{tab:data_tab_1}
%    \begin{tabular}{l|l|l}
%        \hline
%         \textbf{Dataset} & \textbf{\#Data points} &\textbf{\#Features} \\
%        \hline
%        \multicolumn{1}{l|}{\textbf{Stack Overflow}} & \multicolumn{1}{r|}{55,853} &  \multicolumn{1}{r}{28}\\
%
%      \multicolumn{1}{l|}{ \textbf{Mathematics}} &  \multicolumn{1}{r|}{70,336} &  \multicolumn{1}{r}{27}\\
%
%     \multicolumn{1}{l|}{\textbf{Ask Ubuntu}} &   \multicolumn{1}{r|}{7,134} &  \multicolumn{1}{r}{26}\\
%
%      \multicolumn{1}{l|}{\textbf{Super User}}  &  \multicolumn{1}{r|}{10,776} &  \multicolumn{1}{r}{27}\\
%
%
%       \multicolumn{1}{l|}{\textbf{Linux Patch Acceptance Time (Patch) }} &  \multicolumn{1}{r|}{20,000} &  \multicolumn{1}{r}{22}\\
%
%      \multicolumn{1}{l|}{\textbf{Bug-fix Delay Time (Bug-delay)}}   &  \multicolumn{1}{r|}{2,434} &  \multicolumn{1}{r}{23}\\
%
%\multicolumn{1}{l|}{\textbf{Mobile App Rating (App-Rating)}} &  \multicolumn{1}{r|}{7,365} &  \multicolumn{1}{r}{22}\\
%
%        \hline
%    \end{tabular}
%\end{table}
%that pertain to questions, answer, askers, and answerers in the datasets as
\begin{comment}
\noindent\textbf{Q\&A websites data:} We reuse datasets from a prior study by Wang \textit{et al.}~\cite{wang2017}, which investigated the features that potentially impact the needed time to receive an accepted answer to a question on Q\&A websites. The datasets, which were originally collected from the Stack Exchange sites, are comprised of all of the questions that were posted on Stack Overflow in the year 2015 and all the questions ever posted on Mathematics, Ask Ubuntu, and Super User until December 21\textsuperscript{st} 2015. The datasets have 55,853, 70,336, 7,134, 10,776 data points for Stack Overflow, Mathematics, Ask Ubuntu, and Super User, respectively. We use features outlined by Wang \textit{et al.}~\cite{wang2017}. We treat the time it took for a question to get an accepted response as the dependent variable in our study.

\noindent\textbf{Linux patch acceptance time (Patch) data:} We use a dataset from a prior study by Jiang \textit{et al.}~\cite{jiang2013will}. The dataset records the features that impact the acceptance time of patches that are submitted to the Linux kernel's source code. The dataset contains 251,418 data points. We use the patch acceptance time as our dependent variable.


\noindent\textbf{Bug-fix delay time (Bug-delay) data:} We use the dataset from a prior study by Zhang \textit{et al}.~\cite{zhang2012empirical}. The dataset is obtained from the merging of the bug reports that are available in the Bugzilla tracker for three open source projects Mylyn, Platform (runtime provider of Eclipse), and PDE.
%and the data are merged
%From these bug reports, various metrics for each of the bugs reported are extracted such as  severity of the bug, operating system where the bug was found, code metrics associated with these bugs (version of the code before the first change for the reported bug is used), source code changes and fine-grained change type metrics.
The dataset contains 2,435 data points. We use the DelayBeforeChange (DBC), the interval between the time when a bug is assigned to a developer and the time when the developer starts to fix the bug, as the dependent variable of interest in our study.


\noindent\textbf{Mobile app rating (App-rating) data:} We use the dataset from a prior study by Tian \textit{et al.}~\cite{Tian:2015} on various features of 7,365 mobile apps spanning 30 categories. The dataset was collected to understand the features of highly rated mobile apps. We use the rating of the mobile apps as our dependent variable. \
\end{comment}




%\noindent\textbf{Criterion 1: Remove all the questions that are self-answered}\\
%As self-answered questions are often posted for knowledge sharing instead of seeking for an answer, the time to get an accepted answer gets biased by more than just the studied factors. So to avoid this, we remove these data points from our study.\\
%\noindent\textbf{Criterion 2:  Remove questions with missing data}\\
%Some of the factors in our chosen datasets have values missing values due to the inherent nature of the dataset. For instance, some of the questions don't have an accepted answer because some developers who post the question never accept an answer and so on. We consider this values to be missing at random, and as~\cite{mockus2008missing} suggests, we remove those data points from analysis and use only the available data points.\\






==> prestudy.tex <==
%\sw{i think this paragraph and the motivation part could be merged}
%\sw{the motivation looks duplicated with that of introduction, either shorten them or just remove them}

%With the absence of pre-existing class labels, the traditional way of building a classifier on a continuous dependent variable is by artificially introducing a threshold to discretize the continuous dependent variable and assign one class label to the data points that belong to each side of the threshold, respectively.

\begin{comment}
When there are no well-defined rules for determining the threshold for discretization, a variety of previous studies have used median as the discretization threshold~\cite{choi2015machine,iacobucci2015toward,iacobucci2015median,abdelmoez2012bug}. However, using the median as the threshold for discretizing the dependent variable may result in the mislabeling of data points that are close to the median.



To avoid discretization noise, prior studies use the top $x\%$ and bottom $x\%$ of the continuous dependent variable (i.e., extremes shown in Figure~\ref{fig:framework_2}) for assigning class labels~\cite{Tian:2015,peto2008use,wang2017,judd2009learning,abdelwahab2015supervised,abdelmoez2012bug}. While this approach circumvents the discretization noise, it suffers from losing potentially useful information, as it only uses a small portion of the data to build classifiers. Although different studies used different $x\%$'s, there are no clear rules for defining the areas of data that contain most of the discretization noise.


More specifically, as we can see in Table~\ref{tab:framework_tab_1}, on the 7 studied datasets if we consider the $limit$ value as listed in Table~\ref{tab:framework_tab_1} to define the noisy area, on average 25\% of the data across the 7 datasets is considered as the noisy area. For instance, Ask Ubuntu has 7,134 data points in total and 1,880 data points are in the noisy area which makes up 26\% of the data. The removed data might contain useful information which we would miss modeling and more importantly misunderstand the aspects of the data in this region. In summary, much of our observations would be derived from the extremes of the data instead of the overall data.
\end{comment}

In this preliminary study, we seek to understand two important points: 1) whether the data with the discretization noise contains any useful information; 2) whether the discretization noise truly makes the data noisy.
%We accomplish these tasks by employing the framework as described in the Section~\ref{sec:framework}.
%we seek to understand if the data around the median $(median \pm (median * 0.50))$ is the same as data in the top and bottom $20\%$ and whether the model that is built from one region could predict the data points in another region.

%We select $20\%$ as the threshold since many of the previous studies~\cite{judd2009learning,borji2012boosting} use top and bottom $20\%$ for building the classification model that represents the characteristics of the whole dataset.


%\begin{table}
%\centering
%
%    \caption{Statistics about the datasets.}\label{tab:prem_tab_1}
%    \begin{tabular}{l|l|l|l|l}
%        \hline
%         \textbf{Dataset} & \textbf{\# Extremes}  & \textbf{\# Noisy area} &\textbf{\# Size} & \textbf{\%noisy area} \\
%        \hline
%        \multicolumn{1}{l|}{Stack Overflow} & \multicolumn{1}{r|}{22,365}  & \multicolumn{1}{r|}{14,171} &  \multicolumn{1}{r|}{55,853} &  \multicolumn{1}{r}{25}\\
%
%      \multicolumn{1}{l|}{Mathematics} & \multicolumn{1}{r|}{28,151}  & \multicolumn{1}{r|}{19,023} &  \multicolumn{1}{r|}{70,336}&  \multicolumn{1}{r}{27}\\
%     \multicolumn{1}{l|}{Ask Ubuntu} & \multicolumn{1}{r|}{2,848} & \multicolumn{1}{r|}{1,880} & \multicolumn{1}{r|}{7,134}  &  \multicolumn{1}{r}{26}\\
%
%      \multicolumn{1}{l|}{Super User} & \multicolumn{1}{r|}{4,313}  & \multicolumn{1}{r|}{2,759} & \multicolumn{1}{r|}{10,776}  &  \multicolumn{1}{r}{26}\\
%
%
%       \multicolumn{1}{l|}{Patch} & \multicolumn{1}{r|}{8,000} & \multicolumn{1}{r|}{3,743} & \multicolumn{1}{r|}{20,000} &  \multicolumn{1}{r}{19} \\
%
%      \multicolumn{1}{l|}{Bug-delay} & \multicolumn{1}{r|}{974}   & \multicolumn{1}{r|}{537}& \multicolumn{1}{r|}{2,434} &  \multicolumn{1}{r}{22}\\
%
%\multicolumn{1}{l|}{App-rating} & \multicolumn{1}{r|}{2,959}  & \multicolumn{1}{r|}{2,270} & \multicolumn{1}{r|}{7,365}  & \multicolumn{1}{r}{31} \\
%
%        \hline
%    \end{tabular}
%
%
%\end{table}

\begin{table*}
    \centering
    %\scriptsize
\begin{threeparttable}
    \caption{Performance (AUC) of the RFCMs on the different regions of the data.\label{tab:prem_tab_2}}
    \begin{tabular}{l|lllllll}
        \hline
        \textbf{Training data $\rightarrow$ Testing data}& \textbf{SO}& \textbf{MA}& \textbf{AU}& \textbf{SU}& \textbf{Patch}& \textbf{Bug-delay}& \textbf{App-rating}\\
        \hline
%        \textbf{Extremes $\rightarrow$ Extremes} & \multicolumn{1}{r}{0.95}& \multicolumn{1}{r}{0.94}& \multicolumn{1}{r}{0.84}& \multicolumn{1}{r}{0.85} & \multicolumn{1}{r}{0.98} & \multicolumn{1}{r}{0.73} & \multicolumn{1}{r}{0.82}  \\
%        \textbf{Extremes $\rightarrow$ Noisy area} & \multicolumn{1}{r}{0.59} & \multicolumn{1}{r}{0.60}& \multicolumn{1}{r}{0.56}& \multicolumn{1}{r}{0.56} & \multicolumn{1}{r}{0.53}& \multicolumn{1}{r}{0.56}& \multicolumn{1}{r}{0.57}\\
    %    \textbf{Extremes $\rightarrow$ Full data} & \multicolumn{1}{r}{0.77} & \multicolumn{1}{r}{0.77}& \multicolumn{1}{r}{0.66}& \multicolumn{1}{r}{0.68} & \multicolumn{1}{r}{0.73}& \multicolumn{1}{r}{0.64}& \multicolumn{1}{r}{0.67}\\
   %     \textbf{Extremes $\rightarrow$ Full data without noisy area} & \multicolumn{1}{r}{0.85} & \multicolumn{1}{r}{0.84}& \multicolumn{1}{r}{0.70}& \multicolumn{1}{r}{0.74} & \multicolumn{1}{r}{0.80}& \multicolumn{1}{r}{0.67}& \multicolumn{1}{r}{0.74}\\
        \textbf{Noisy area $\rightarrow$ Extremes} & \multicolumn{1}{r}{0.89} & \multicolumn{1}{r}{0.88}& \multicolumn{1}{r}{0.68}& \multicolumn{1}{r}{0.70} & \multicolumn{1}{r}{0.80}& \multicolumn{1}{r}{0.57}& \multicolumn{1}{r}{0.61}\\
        \textbf{Noisy area $\rightarrow$ Noisy area} & \multicolumn{1}{r}{0.57}& \multicolumn{1}{r}{0.57}& \multicolumn{1}{r}{0.53}& \multicolumn{1}{r}{0.52}& \multicolumn{1}{r}{0.80} & \multicolumn{1}{r}{0.57} & \multicolumn{1}{r}{0.55}   \\

        \hline

   %     \textbf{Noisy area $\rightarrow$ Full data} & \multicolumn{1}{r}{0.57}& \multicolumn{1}{r}{0.57}& \multicolumn{1}{r}{0.53}& \multicolumn{1}{r}{0.52}& \multicolumn{1}{r}{0.80} & \multicolumn{1}{r}{0.57} & \multicolumn{1}{r}{0.55}   \\
  %      \textbf{Noisy area $\rightarrow$ Full data without noisy area} & \multicolumn{1}{r}{0.57}& \multicolumn{1}{r}{0.57}& \multicolumn{1}{r}{0.53}& \multicolumn{1}{r}{0.52}& \multicolumn{1}{r}{0.80} & \multicolumn{1}{r}{0.56} & \multicolumn{1}{r}{0.58}   \\
  \textbf{Full data without noisy area$\rightarrow$ Full data without noisy area} & \multicolumn{1}{r}{0.82}& \multicolumn{1}{r}{0.82}& \multicolumn{1}{r}{0.67}& \multicolumn{1}{r}{0.70}& \multicolumn{1}{r}{0.95} & \multicolumn{1}{r}{0.70} & \multicolumn{1}{r}{0.78}\\
 \textbf{Full data$\rightarrow$ Full data} & \multicolumn{1}{r}{0.78}& \multicolumn{1}{r}{0.77}& \multicolumn{1}{r}{0.65}& \multicolumn{1}{r}{0.68}& \multicolumn{1}{r}{0.92} & \multicolumn{1}{r}{0.68} & \multicolumn{1}{r}{0.72}\\

        \hline
    \end{tabular}
        \begin{tablenotes}
            \small
            \item  SO - Stack Overflow, MA - Mathematics, AU - Ask Ubuntu, SU - Super User
        \end{tablenotes}
\end{threeparttable}

\end{table*}
\noindent\textbf{Approach:} We aim to understand if the noisy area of the dataset contains useful information. To do so, we train a classifier on the noisy area and test it on the data from the extremes for each of the studied datasets. The extremes and the noisy area in the dataset are as shown in Figure~\ref{fig:framework_2}. We use the framework that is outlined in Figure~\ref{fig:fig1}. A good performance (we evaluate on only AUC value for this section, as it would make evaluation on multiple measures cumbersome) for the RFCMs that are constructed in the noisy area on the extremes indicates that the data of the noisy area contains useful information that should not be removed cursorily.

%We first sort the dependent variable, then discretize the data and label them as outlined in Section~\ref{sec:framework}. We then
To evaluate if the data in the noisy area is indeed noisy, we train our RFCMs on the noisy area and test them on the out-of-sample test set from the noisy area. The limits that are used to define the noisy area are as outlined in Table~\ref{tab:framework_tab_1}. A bad performance for the constructed RFCMs on the noisy area indicates that the data in the noisy area indeed contains a large amount of noise. That is to say the noise would impact the performance of a classifier even if the RFCM was constructed on the noisy area and it does contain useful information.
%the noise that is present, might impact
%We validate the generated AUC results through a 100 out-of-sample bootstrap validation.
Prior studies~\cite{Tian:2015,peto2008use,wang2017,judd2009learning,abdelwahab2015supervised,abdelmoez2012bug} used different $x$ for defining the extremes. As the choice of $x$ for defining the extremes is not clear-cut, we set $x=20$ to define extremes in this study.
%But our framework allows for different values of x to be specified for defining the extremes in a dataset.


%As we mentioned before, prior studies by Tian~\textit{\etal} and Peto~\textit{\etal}~\cite{Tian:2015,peto2008use} use different $x\%$ to define extremes in their study. For instance, Tian~\textit{\etal}~\cite{Tian:2015} uses $x=10\%$ and uses the top $10\%$ and bottom $10\%$ of the continuous dependent variable. They use the independent features that are associated with the top and bottom $10\%$ of the dependent variable as the extremes dataset along with the dependent variable and build their classifiers on the extremes. Whereas other studies~\cite{peto2008use} use a different value for $x$. As the choice of $x$ for defining the extremes is not clear-cut, we set $x=20$ to define extreme in this study. But our framework allows for different values of x to be specified for defining the extremes in a dataset.


\noindent\textbf{Findings:}
%\sw{i think we can drop this. the following two findings are enough to support our points,1 noise is noise,2 noise has useful info. the conclusion is not true, it is not extreme can capture the sig of noise, but the noise data is too complex and hard to divide. even itself can't predict.\gopi{Fixed}}
%\textbf{RFCMs that are trained on the extremes of the data cannot predict the data in the noisy area well.} As we observe from Figure~\ref{fig:prem_1}, the performance of RFCMs that are trained on the extremes of the different datasets have performance that is only slightly better than random guessing (i.e., the median AUC value does not exceed $0.60$ in all the datasets)~\cite{wigton1986transportability} on the noisy area across all the datasets.The Figure~\ref{fig:prem_1} clearly highlights that the data in the extremes alone are incapable of modeling the noisy area and we need to consider the data in the noisy area too since it makes up for one-fourth of the data.
\textbf{The noisy area contains useful information that might help improve the performance of RFCMs.} From Table~\ref{tab:prem_tab_2}, we observe that the RFCMs that are trained on the noisy area perform relatively well on the extremes for 4 out of the 7 studied datasets. Three datasets have an AUC that is larger than 0.7. For instance, in the Stack Overflow dataset, the RFCMs trained on the noisy area have an AUC of 0.89 in the extremes. While there is a drop in performance when compared to the classifiers that are trained on extremes themselves, an AUC of 0.89 is still a very high AUC indicating that the constructed classifier performs well. The drop in performance is expected as the noisy area may have characteristics that are different from the extremes area or might contain noise.


%RFCMs that are trained on the noisy area having good performance on the extremes suggests that researchers cannot remove the noise area cursorily.
%The situation also highlights a need for a framework, like our framework to evaluate the usefulness of the data in the noisy area.
%We can observe the poor performance for an RFCM that is trained on the noisy area and tested on data from the extremes in Figure~\ref{fig:prem_1}.
% We also provide the performance measure (AUC) of an RFCMs that is trained and tested on the whole dataset and an RFCM that is trained and tested on the dataset without the noisy area in Table~\ref{tab:prem_tab_2} for all the studied datasets.


%\begin{figure}
%    \includegraphics[width=\linewidth]{figures/prem_1.pdf}
%    \caption{Poor performance of RFCMs that are trained on extremes and tested on the noisy area across the studied datasets.}
%    \label{fig:prem_1}

%\end{figure}




%we see a consistent increase in performance for the RFCMs that are trained on extremes, over the RFCMs trained on noisy area. Such a phenomenon indicates that data in the noisy area might potentially be harming the performance of the classifiers. The results are in agreement with many prior studies about class noise~\cite{zhu2004class,zhu2003eliminating}, which show the impact of class noise on the performance of classifiers. This phenomenon holds true for our discretization noise as well.
\textbf{Although the noisy area does contain useful information, the discretization noise still affects the performance of an RFCM.} From Table~\ref{tab:prem_tab_2} shows that an RFCM that is trained on the noisy area performs poorly on its own out-of-sample test set in the noisy area (Except for the Patch dataset, this is due to the complexity of the noisy area of Patch dataset compared to other datasets. More details are presented in Section~\ref{sec:disc}). Such a low performance for RFCMs that are trained on the noisy area indicates that while the noisy area does contain useful information, the discretization noise in the noisy area still affects the performance of RFCMs.

With these contradicting points both in favor and against the inclusion of data in the noisy area, in the remainder of this study, we seek to study the impact of discretization noise on the performance of RFCMs using the framework that we proposed in Section~\ref{sec:framework}. We also seek to understand the impact of discretization noise on the interpretation of RFCMs in the Section~\ref{sec:rqs}.


